Involutive moving frames II; The Lie-Tresse theorem

This paper continues the project, begun in \cite{IMF}, of harmonizing Cartan's classical equivalence method and the modern equivariant moving frame in a framework dubbed \emph{involutive moving frames}. As an attestation of the fruitfulness of our framework, we obtain a new, constructive and intuitive proof of the Lie-Tresse theorem (Fundamental basis theorem) and a first general upper bound on the minimal number of generating differential invariants for Lie pseudo-groups. Further, we demonstrate the computational advantages of this framework by studying the equivalence problem for first order PDE in two independent variables and one dependent variable under point transformations.

==> ev_free.tex <==
\section{Appendix: Eventually free Lie pseudo-groups}

As previously mentioned, the foundational work, \cite{OP-2008, OP-2009}, on the equivariant moving frame for pseudo-groups focused on pseudo-group actions that were \emph{eventually free}, meaning that at some order, the groupoid action, see (\ref{eq:hatw}), of $\H_q$ on some subset $\V_q\subset J^q(\E)$ was free. Equivalently, each group parameter of order $\leq q$ can be normalized in the lifted invariants $\UhaJ$, $|J|\leq q$, restricted to $\V_q$. The key result in \cite{OP-2009}, dubbed \emph{persistence of freeness}, says that if the action is free at order $q$ in $\V_q$, it is also free at order $q+1$ on the pre-image $(\pi^{q+1}_q)^{-1}(\V_q)$ where $\pi^{q+1}_q:J^{q+1}(\E)\to J^q(\E)$ is the canonical projection. In this section we prove that eventually free actions are quasi-horizontal and that persistence of freeness is a trivial consequence thereof. 

%There is a remarkable contrast between the complexity of the proof of persistence of freeness from \cite{olver09} and the following, almost trivial, proof. 

As a quick warm up for the general case, consider a Lie pseudo-group acting on graphs of maps $x\mapsto u(x)$, $x\in\R$, in $\R^2$. The total derivative on $J^\infty(\R^2\to\R)$ is
\[
D_x=\pder{x}+\sum u_{k+1}\pder{u_k},
\]
where $u_k$ is the $k\th$ $x$-derivative of u. The first prolongation of a map $\p(z)=\p(x,u)=(X,U)=Z$ is
\[
\Uh_X=\frac{D_xU}{D_xX}=\frac{U_x+u_xU_u}{X_x+u_xX_u},
\]
but notice that the nominator and denominator are the $\dis\frac{\partial}{\partial y}$ derivatives of $U$ and $X$ in flat coordinates for the graph of $x\mapsto u(x)$ since, on the graph of $u$,
\[
\dis\frac{\partial}{\partial y}=\dis\frac{\partial}{\partial x}+u_x\dis\frac{\partial}{\partial u}.
\]

It is easily seen that in general, on the graph of $x\mapsto u(x)$, we have that
\beq\label{eq:dy}
\frac{d^k}{dy^k}\p=D_x^k\p.
\eeq
Defining
\[
D_{\mathrm{X}}=\frac{1}{D_xX}D_x,
\]
the higher order prolongations of $\p$ are
\[
\Uh_k=D_{\mathrm{X}}^kU,
\]
which are functions of the $y$-derivatives of $\p$ only. In arbitrary many variables, $n+m$, for $\E=\X\times\U$, and a local diffeomorphism $\p(x,u)=(X,U)$, the formulas for $\Uh_J$, restricted to a graph of $x\mapsto u(x)$, become rather complicated but they too are functions of the expressions
\[
\frac{\partial^{|K|}}{\partial y^K}\p^a=D^K\p^a,\quad K\in\mathbb{Z}_{\geq0}^n,
\]
where
\[
\frac{\partial}{\partial y^i}=\frac{\partial}{\partial x^i}+u\av_i\frac{\partial}{\partial u\av}.
\]
%\]
%and
%\[
%D_{x^i}=\partial
%\]
%which, satisfies, on the graph of $x\mapsto u(x)$,
%\beq\lalbel{eq:partialy}
%\frac{d^k}{dy^k}Z=D_x^kZ.
%\eeq
%To see why, let $A$ be the $n\times n$ matrix with entries 
%\[
%A_{ij}=\partial_{y^i}X^j=X^j_i+u\av_iX^j_\alpha.
%\]
%(Here, $ij$ refers to line $i$ and column $j$.) Then, letting $A^{ij}$ be the components of $A^{-1}$, we have
%\[
%\Uha_i=A^{ji}\partial_{y^j}U\av. 
%\]
%Since $A^{ji}$ is a rational function in the components of $A$, $\Uha_i$ is a function of $\partial_{y^i}Z^a$. In general, setting $D_{\mathrm{X}^i}=A^{ji}\partial_{y^j}$, we have
%\[
%\UhaJ=D_{\mathrm{X}^J}U\av,
%\]
%where $D_{\mathrm{X}^J}=(D_{\mathrm{X}^1})^{J_1}\dots (D_{\mathrm{X}^n})^{J_n}$ and $J=(J_1, \ldots, J_n)\in\mathbb{Z}_{\geq0}^n$, which is clearly a function of $\dis \frac{\partial^{|K|}}{\partial y^K}Z^a$, $|K|\leq|J|$. 

%Let us write $\Zb^a_K$ for the expressions $\dis \frac{\partial^{|K|}}{\partial y^K}Z^a$ in what follows. 
 
Now assume the action of $\H$ on $\E$ is free at order $q$ in $\V_q\subset J^q(\E)$ and $j^qu\resx \in\V_q$. Let $x\mapsto u(x)$ be a representing map with $q$-jet $j^qu\resx$ at $x$ and such that the entire $q$ jet $j^qu$ lies in $\V_q$. Freeness means that it is possible to solve for every group parameter in a set of equations (restricted to $x\mapsto u(x)$) of the form
\beq\label{eq:ucon}
\Uh^{\alpha_r}_{J^r}=c^{\alpha_r}_{J^r}=\text{constant},
\eeq
for $1\leq r\leq \delta(q)$, where $\delta(q)$ is equal to the number of parametric derivatives in $\H_q$. Write the determining equations in flat $(y,w)$ coordinates w.r.t. $x\mapsto u(x)$. We shall prove that $\H$ is necessarily quasi-horizontal. We write $\pmb{Y}^{(q)}$ for those pseudo-group jet coordinates $Z^a_K$, $|K|\leq q$, that are pure $y$-derivatives and $\pmb{W}^{(q)}$ for those $Z^a_K$, $|K|\leq q$ that are nor. We consider two sets of equations; the determining equations for $\H$ of order $\leq q$ and (\ref{eq:ucon}), in flat coordinates for $u$. These can be written
\begin{align*}
F(z,Z, \pmb{Y}^{(q)}, \pmb{W}^{(q)})&=0,\\
G(z, Z, \pmb{Y}^{(q)})&=0,
\end{align*}
since (\ref{eq:ucon}) only involve $\pmb{Y}^{(q)}$. The fact that this system can be uniquely solved for \emph{all} $\pmb{Y}^{(q)}$ and $\pmb{W}^{(q)}$ directly implies that 
\[
F(z, Z, \pmb{Y}^{(q)}, \pmb{W}^{(q)})=0
\]
can be solved for $\pmb{W}^{(q)}$. In particular, \emph{each} pseudo-group jet involving a $w$-derivative can be taken as principal. Thus, eventually free Lie pseudo-group actions are quasi-horizontal and they have horizontal order equal to the order of the pseudo-group. In addition, each pseudo-group jet involving a $u^\alpha$-derivative can be taken as principal. The free pseudo-groups have therefore are rather special structure.

\begin{theorem}\label{thm:efqh}
Let $\H$ be a $t^*$ order, eventually free Lie pseudo-group acting on the bundle $\E\to\X$. Then $\H$ is quasi-horizontal and all pseudo-group parameters can be taken to be pure $\X$ derivatives.
\end{theorem}

\begin{Ex}\label{ex:stab}
Consider the Lie group action
\[
(x, u)\mapsto (\lambda x + a, \lambda^{k+1}u + P_k(x)),\quad \lambda>0,
\]
where $P_k(x)$ is an arbitrary polynomial of order $k$. The determining equations for this pseudo group are
\[
X_u=0,~~X_{xx}=0,~~ U_u=X_x^{k+1},~~ \frac{\partial^{k+1}}{\partial x^{k+1}}U=0.
\]
Notice that, in accordance with the above theorem, \emph{each} pseudo-group jet involving a $u$-derivative can be taken as principal. The order of the pseudo-group is $k+1$.
\end{Ex}

We can now present a rather trivial proof of \emph{persistence of freeness} of Lie pseudo-groups. Let $j^qu\resx\in\V_q\subset J^q(\E)$ lie in a set $\V_q$ on which $\H_q$ acts freely, as above. In flat coordinates w.r.t. a representing map $x\mapsto u(x)$, each pseudo-group jet involving a $w$ derivative can be taken as principal. Let us denote the pseudo-group jets coordinates in $\pmb{Y}^{(q)}$ that have order equal to $q$ by $\pmb{Y}^q$. Then in the determining equations $F^{(q)}(z, Z^{(q)})=0$, ignoring those equations with principal derivatives having a $w$-derivatives and those of order less than $q$, we have some subset of $q\th$ order determining equations $\bar{F}^{(q)}(z, \pmb{Y}^{q})=0$ that only involve pure $y$-derivatives of order $q$. Then the $y$-prolongations
\[
\left(\partial_{y_1}\bar{F}^{(q)}\right)(z, \pmb{Y}^{q+1})=0,\ldots, \left(\partial_{y_n}\bar{F}^{(q)}\right)(z, \pmb{Y}^{q+1})=0
\]
give a system $\bar{F}^{(q+1)}(z, \pmb{Y}^{q+1})=0$ of determining equations of order $q+1$ that involve only pseudo-group jets of pure $y$-derivatives.

By freeness, on $\V_q$, there is a collection $\Uh^{\alpha_s}_{J^s}$, $1\leq s\leq \delta^*(q)$, of lifted invariants with $|J^s|=q$, from which all $q\th$ order parametric derivatives can be normalized, where $\delta^*(q)$ is the number of pseudo-group parameters of order exactly $q$. That is, the collection $\Uh^{\alpha_s}_{J^s}$, $1\leq s\leq \delta^*(q)$, is full rank in the $q\th$ order parametric derivatives (all of which are pure $y$-derivatives since $\H$ is eventually free). Hence, the set of functions on $\Ht^q$,
\beq\label{eq:fuh}
\left\{\bar{F}^{(q)}(z,  \pmb{Y}^{q}), \Uh^{\alpha_s}_{J^s}\right\}\restrict{1\leq i\leq \delta^*(q)}
\eeq
is full rank in the pseudo-group jets $\pmb{Y}^{q}$ when evaluated at jets in $\V_q$. Now, for any lifted invariant $\UhaJ$, the two collections (once evaluated at $j^qu\resx$)
\beq\label{eq:2col}
\aligned
\{D_{X^i}\UhaJ\}_{1\leq i\leq n},\quad \{\partial_{y_i}\UhaJ\}_{1\leq i\leq n}
\endaligned
\eeq
are invertible linear combinations of each other with coefficients depending on first order jets. Therefore the two collections (\ref{eq:2col}) are equal in rank in the top order pseudo-group jets. Going back to (\ref{eq:fuh}), this means that prolonging all functions in (\ref{eq:fuh}) w.r.t $\partial_{y_i}$ for $1\leq i\leq n$ will give a collection having the same rank in the $\pmb{Y}^{q+1}$ as the system
\beq\label{eq:fuh2}
\left\{\bar{F}^{(q+1)}(z,  \pmb{Y}^{q+1}), \Uh^{\alpha_s}_{J^s, j}\right\}\restrict{1\leq i\leq \delta^*(q), 1\leq j\leq n}.
\eeq
But since (\ref{eq:fuh}) was full rank in $\pmb{Y}^q$, its prolongation w.r.t. the $y$ variables will be full rank in $\pmb{Y}^{q+1}$. Since (\ref{eq:fuh2}) has the same rank in $\pmb{Y}^{q+1}$ we have proved persistence of freeness.

%applying $\partial_{y_i}$ to all expressions  In particular  
%Now assume $S$ is the graph of $u(x)$ and $\Sb$ is the graph of $\ub(\xb)$. An equivalence map $\p(x, u)=(X(x, u), U(x, u))\in\H$ from $S$ to $\Sb$ will satisfy the determining equations of $\H$ as well as the equivalence conditions
%\beq\label{eq:eqcond}
%\Ua(y, 0)=\uba(X(y,0)).
%\eeq
%Notice that differentiating this w.r.t. $y_i$ gives
%\[
%\Ua_{y_i}(y,0)=\sum_j\uba_j((X(y,0))X^j_{y_i}(y,0),
%\]
%doing this for all the $y_i$, we find the equivalent system
%\[
%\Uha_{X^i}(y,0)=\uba_i(X(y,0)).
%\]
%And so, not surprisingly, prolonging the equivalence condition (\ref{eq:eqcond}) just brings us to the restriction of the prolongation formulas to $S$. For an arbitrary $J\in\Nz^n$ we find, after prolonging (\ref{eq:eqcond}), $|J|$ times,
%\beq\label{eq:eqcondJ}
%\UhaJ(y,0)=\uba_J(X(y,0)).
%\eeq
%
%Now let $F_p(z, Z^{(p)})=0$ be the $p\th$ order determining equations of $\H$ and assume the action of $\H_p$ on $\V_p\subset J^p(\E)$ is free. If $j\resx^p  u$ and $j\resxb^p \ub$ both lie in $\V_p$, freeness at order $p$ means that there are pairs $(\alpha_1, J^1), \ldots, (\alpha_t, J^t)$ such that the system
%\begin{align*}
%F(z, Z^{(p)})&=0,\\
%\Uh^{\alpha_i}_{J^i}(y,0)&=\ub^{\alpha_i}_{J^i}(X(y,0)), \quad 1\leq i\leq t,
%\end{align*} 
%can be solved for all pseudo-group jet coordinates above first order. Here, $t$ is the number of parametric derivatives/group parameters in $\H$. We can therefore write this system in an equivalent form
%\begin{align*}
%F_p(z, Z^{(p)})&=0,\\
%Z^{a_i}_{K^i}(y,0)&=G^i(y, Z(y,0)),\quad 1\leq i\leq t,
%\end{align*}
%for some functions $F^i$ and multi-indices $K^i\in\Nz^n$, where, in the above equations we can solve for all pseudo-group jets of order $\leq p$. Now, simply prolonging the determining equations $F_p(z, z^{(p)})=0$ and prolonging the second set of equations w.r.t. the $y$-variables will give a system where we can solve for all pseudo-group jets of order $\leq p+1$. In other words, the prolonged action of $\H_p$ on $\V_p$ is also free. This gives a simple proof of persistence of freeness of Lie pseudo-groups!

% The expressions $\UhaJ$ only involve $y$ derivatives and we shall prove that, then the group parameters of $\H$ in flat coordinates for any $u$ such that $j\resx^pu\in\V_p$ can only involve $y$ derivatives. Said differently, since the flat coordinate change is fiber preserving in $\E$, $\H$ must be quasi-horizontal of order 1. We pause to make a record of this fact. 
%
%
%
%
%
%A Lie pseudo-group of transformations on $\E=\X\times\U$ is said to bee \emph{free} at order $p$, at some point $z^{(p)}\resx\in J^p(\E)$, if the action of the groupoid $\G_p$ on $J^p(\E)$ is free at $z^{(p)}\resx$. Equivalently, every group parameter of $\G$ up to order $p$ can be normalized from the lifted invariants $\UhaJ$, $|J|\leq p$. But notice that since all the lifted invariants are functions of the $\ZbaK$, we can only really normalize these. For example, if $\ZbaK$ depends on two group parameters that do not appear in any other $\Zb^b_N$, then there is no hope of normalizing both group parameters. This means that a necessary condition for freeness at order $p$ is that the collection of $\ZbaK\restrict{\G}$, $K\in\Nn$, $|K|\leq p$, have the same rank as the collection $Z^a_L\restrict{\G}$, $L\in\Nz^{n+m}$, $|L|\leq p$. Obviously, the latter collection has rank equal to the number of parametric derivatives of order $\leq p$ and so we obtain some obvious restrictions on the size of the formal solution space of $\G$ in order for it to become free. For example, when $\G$ is given in involutive form it can not have any parametric derivatives of class greater that $n$. Further, it may not have more than $m$ parametric derivatives of class $n$.
% 
%\begin{theorem}\label{the:eventual}
%Every eventually free Lie pseudo-group $\G$ is hypo-projective.
%\end{theorem}
%
%The proof of this theorem essentially boils down to the following simple, linear-algebraic, lemma. For a smooth function $f(x,y,z)$, from $\R^a\times\R^b\times\R^c\to\R^d$, we denote the submatrix of the Jacobian of $f$ consisting of the columns corresponding to differentiation with respect to, for example, the $x$ variables by $\nabla_xf$. The matrix of columns corresponding to differentiation with respect to the $x$ and $y$ variables is denoted $\nabla_{x,y}$ and so on. We say that $f$ is \emph{full rank} in the $x$ variables if $\nabla_xf$ is full rank, and so on. 

%\begin{lemma}\label{le:ybar}
%Let $\bar{y}=f(x,y)$ for a smooth function $f:\R^a\times\R^b\to\R^c$, where $x\in\R^a$, $y\in\R^b$, $\bar{y}\in\R^c$ and $c\leq b$. Let $G:\R^a\times\R^c\to\R^c$ and assume the following holds, for some smooth $g:\R^a\to\R^b$,
%\[
%G(x,\bar{y})=0~~\Leftrightarrow~~ y=g(x).
%\]
%Then $b=c$ and there exists a smooth function $h(x,\bar{y})$ such that $y=h(x,\bar{y})$. 
%\end{lemma}
%
%\begin{proof}[Proof of lemma]
%Since we can solve for all $y$ in $G(x,\bar{y})=G(x,f(x,y))=0$ the function 
%\[
%(x,y)\mapsto G(x,f(x,y))
%\]
%must have full rank with respect to $y$, that is $\nabla_yG$ has full rank $b$. Since $\nabla_yG$ has only $c$ rows, we must have $c=b$. The matrix $\nabla_yG$ is then an invertible $b\times b$ matrix. By the chain rule we have
%\[
%\nabla_yG=\nabla_{\bar{y}}G\cdot\nabla_yf
%\]
%and $\nabla_{\bar{y}}G$ must have rank $b$ and therefore be invertible. We then have that
%\[
%\nabla_yf=\nabla_yG\cdot(\nabla_{\bar{y}}G)^{-1}
%\] 
%is invertible. We then have that the smooth map
%\[
%(x,y)\mapsto (x,\bar{y})=(x, f(x,y)) 
%\]
%is invertible and its inverse provides a smooth function $h$ such that 
%\[
%y=h(x,\bar{y}). 
%\]
%
%\end{proof}


%\begin{lemma}
%Let $x\in\R^a$, $y\in\R^b$ and $z\in\R^c$ and let $\bar{y}=f_1(x,y)$, for a smooth function $f_1:\R^a\times\R^b\to\R^{b'}$, and let $\zb=f_2(x,y,z)$, for a smooth function $f_2:\R^a\times\R^b\times\R^c\to c'$ and for $b'\leq b$ and $c'\leq c$. Let $G:\R^a\times\R^b\times\R^c\to\R^{b'+c'}$ and assume the following holds, for some smooth $g:\R^a\to\R^{b+c}$,
%\[
%G(x,\bar{y}, \zb)=0~~\Leftrightarrow~~ (y, z)=g(x).
%\]
%Then $b=b'$ and $c=c'$ and there exists a smooth function $h(x,\bar{y})$, that is full rank in the $\bar{y}$ variable, such that $y=h(x,\bar{y})$. 
%\end{lemma}
%
%\begin{proof}[Proof of lemma]
%Since we can solve for all $y$ and $z$ in $G(x,\bar{y}, \zb)=G(x,f_1(x,y),f_2(x,y,z) )=0$, by the rank theorem, the function 
%\[
%(x,y, z)\mapsto G(x,f_1(x,y), f_2(x,y,z))
%\]
%must have full rank with respect to $y$ and $z$. That is, $\nabla_{y, z}G$ has full rank $b+c$. Since $\nabla_{y,z}G$ has only $b'+c'\leq b+c$ rows and since $b'\leq b$ and $c'\leq c$, this implies that $b'=b$ and $c'=c$. By the chain rule we have
%\beq\label{y,z}
%\nabla_{y,z}G=\left[\nabla_{\bar{y}}G\cdot\nabla_yf_1+\nabla_{\zb}G\cdot\nabla_yf_2~|~\nabla_{\zb}G\cdot\nabla_zf_2\right],
%\eeq
%where $|$ separates the first $b$ columns from the last $c$. Since this matrix is full rank (note that this is then an invertible square matrix), the last $c$ columns, $\nabla_{\zb}G\cdot\nabla_zf_2$ must be full rank $c$. This means that $\nabla_{\zb} G$ must have full rank $c$. We can perform a ``Gaussian elimination'' on the first $b$ columns using the full rank $\nabla_{\zb} G$ to see that the matrix
%\[
%\left[\nabla_{\bar{y}}G\cdot\nabla_yf_1~|~\nabla_{\zb}G\cdot\nabla_zf_2\right]
%\]
%has full rank $b+c$ and, by the same arguments as above, that $\nabla_{\bar{y}}G$ is full rank $b$. We have then showed that $\nabla_{\yb,\zb}G$ is an invertible matrix, just like $\nabla_{y,z}G$. We can write (\ref{y,z}) as the matrix product
%\[
%\nabla_{y,z}G=\nabla_{\yb,\zb}G\cdot \bbm \nabla_yf_1 & 0 \\ \nabla_yf_2 & \nabla_zf_2\ebm\nabla_{\yb, \zb}G\cdot\nabla_{y,z}(f_1,f_2),
%\]
%where $(f_1,f_2)(x,y,z)=(f_1(x,y), f_2(x,y,z))$. Equivalently,
%\[
%\nabla_{y,z}G\cdot(\nabla_{\yb,\zb}G)^{-1} = \nabla_{y,z}(f_1,f_2)
%\]
%and so $\nabla_{y,z}(f_1, f_2)$ is invertible. But this means that the smooth map
%\[
%(x,y,z)\mapsto(x,\yb,\zb)=(x,f_1(x,y), f_2(x,y,z))
%\]
%is invertible and, by the structure of $f_1$ and $f_2$, this inverse will provide a smooth map, full rank in $y$, such that $\yb=h(x,y)$.
%
%\end{proof}
%
%\begin{proof}[Proof of Theorem \ref{the:eventual}]
%We shall prove a stronger result, namely that if all parametric derivatives of $\G$ of order exactly $p$ can be normalized then $\G$ is hypo-projective of order $p$. It is no restriction to assume that $\G_p$ is formally integrable. Let $t$ be the minimal number such that all group parameters of order $p$ can be normalized by normalizing lifted invariants $\UhaJ$, $|J|\leq t$, and assume for simplicity that they were all normalized to zero. In order to apply the preceding lemma, we set $y\in\R^b$ as the group parameters of order $p$, and $\bar{y}\in\R^{b'}$ a maximal collection of $\ZbaK\restrict{\G}$, $|K|=p$, that is full rank in $y$. This means that for any $\Zb^b_N$, $|N|=p$, not in $\yb$ there is a function $f$ such that $\Zb^b_N-f(\yb)$ is not a function of $y$ but only of group parameters of strictly lower order than $p$ and submanifold jet coordinates on $J^p(\E)$. It can well happen that on our way to normalizing all $p\th$ order group parameters, $y$, we will have to normalize some higher order group parameters also. Denote by $z\in\R^c$ the collection of these normalized higher order group parameters and set $\zb=z$. Finally, denote by $x\in\R^a$, all group parameters of order strictly lower than $p$ and the submanifold jet coordinates on $J^t(\E)$. Now set $G(x,\yb, \zb)$ as the collection of all the lifted invariants, $\UhaJ$, $|J|\leq t$, that we normalize before having normalized all the $y$. Then, applying the preceding lemma, we can write 
%\[
%y=h(x,\yb),
%\]
%and $b=b'$. This means that the number of parametric derivatives in the rectified coordinates of order $p$ that are pure $\xb$-derivatives, $b'$, contains \emph{all} $b$ parametric derivatives of order $p$. This proves the theorem. 
%will
%Consider the collection of those lifted invariants $\UhaJ$, $|J|=p$, from whence all the $y$ can be normalized. For simplicity assume they can be normalized to zero and let $G(x,y)$ be this collection of lifted invariants. Then Lemma \ref{le:ybar} says simply that each group parameter of order $p$ can be written as a function of the $\bar{y}$ and $x$. But this means that when we switch to rectified coordinates we can replace each parametric derivative for $\G$ by $\bar{y}$ and some lower order parametric derivatives. Assuming $\G$ is written in solved form,
%\[
%Z^a_L=\Phi^a_L(x,u, \ldots,\text{\pds}, \ldots),
%\]
%we can replace each parametric derivative on the right hand side by a pure $\xb$-derivative. Since $\partial_u=\partial_{\ub}$ every principal derivative involving $u$-derivatives will involve a $\ub$-derivative in rectified coordinates. Furthermore, by definition of $\bar{y}$, each $\dis\frac{\partial^{|K|}}{\partial\xb^K}Z^a$, whether it is part of $\bar{y}$ or not can be written as a combination of $\bar{y}$ and lower order group parameters and submanifold-jet coordinates, i.e. of $\bar{y}$ and $x$. This clearly demonstrates that we can choose a representation of $\G_p$ in the rectified coordinates where all $p\th$ order group parameters are pure $\xb$-derivatives. Since $\G_p$ is formally integrable this means that all $p\th$ order group parameters of $\G$ are pure $\xb$-derivatives.
%\end{proof}
%
%If we can normalize all $p\th$ order group parameters from the lifted invariants $\UhaJ\resS$, then $\G$ is hypo-projective and by Theorem \ref{the:extension} a map $f_p:S\to\G_p$ that annihilates all Maurer-Cartan forms can be uniquely integrated to a pseudo-group element. We say that $\G$ is $p$-free if all $p\th$ order group parameters can be normalized. We now turn our attention to partial moving frames and to applying the fundamental Theorem \ref{GcoX} to solve the equivalence problem of submanifolds in $\E$ under an eventually free Lie pseudo-group.
%
%Let $S$ and $\Sb$ be two submanifolds of $\E$ that are the graphs of two functions $u,\ub:\X\to\U$ and let $s:S\to\G_p\irestrict{0}$ and $\sb:\Sb\to\G_p\irestrict{0}$. (For simplicity we have assumed that all target variables can be normalized to zero.) If a pseudo-group element $\p\in\G$ maps $s$ to $\sb$, $R_\p\cdot s=\sb$, and then also $S$ to $\Sb$, then $\p$ also preserves \emph{all} restricted lifted invariants
%\beq\label{eq:lifted}
%R_\p^*\left(\UhaJ\restrict{\sb}\right)=\UhaJ\ress,\quad|J|\leq p. 
%\eeq
%As before, we choose the maps $s$ and $\sb$ such that (as many as possible) lifted invariants (or combinations thereof) are constant when restricted to $s$ and $\sb$. An important observation is that if $S$ and $\Sb$ are indeed congruent then \emph{all the same} lifted invariants can be normalized when restricted to $S$ and $\Sb$. This is because the lifted invariants agree on $S$ and $\Sb$, see (\ref{eq:lifted}). If we are lucky, after normalizing enough lifted invariants, the problem of building the subsection $f_p$ of $\G_p\overset{\sigma}{\to}\E$ becomes attainable. One special case is when the pseudo-group action is $p$-free on $S$ on $\Sb$. In this case, we can normalize all $p\th$ order group parameters, leading to a partial moving frame $\B_p\subset\G_p\iresn$ on which $\muaL$, $|L|<p$ form a bona-fide right-invariant \emph{coframe}. The congruence problem of $S$ and $\Sb$ now amounts to, by Theorem \ref{GcoX}, finding subsections $s\resS$ and $\sb\restrict{\Sb}$ of $\B_p$ and a subsection $f_p\resS$ of $\G_p$ such that $R_{f_p}\cdot s =\sb$. Since $\G$ is $p$-free this can be handled by finite dimensional means. Consider the restriction of the partial moving frame $\B_p$ to $S$ and $\Sb$, $\B^S_p$ and $\B_p^{\Sb}$ and an equivalence map $\Lambda:\B_p^S\to\B_p^{\Sb}$ that preserves the right-invariant coframe $\muaL$, $|L|<p$. I claim that $\Lambda=R_{f_p}$, for some subsection $f_p\resS$ of $\G_p$ that annihilates the contact codistribution. To see why, choose \emph{any} section $s$ of $\B_p^S\overset{\sigma}{\to}S$ and consider the image $\Lambda(s(S))$. Since $\Lambda$ preserves the horizontal forms $\oa$, $\Lambda(s(S))$ is the image of a section $\sb$ of $\B^{\Sb}_p\overset{\sigma}{\to}\Sb$. By Theorem \ref{GcoX} $\Lambda\restrict{s(S)}$ must have the form $R_{f_{p}}$ for a subsection $f_p$ but the map $\Lambda\cdot \left(R_{f_p}\right)^{-1}:\B_p^S\to\B^S_p$ preserves the coframe $\muaL$, $|L|<p$, and fixes the section $s$. By the Frobenius theorem such a map must be the identity, so $\Lambda=R_{f_p}$. The subsection $f_p$ can be \emph{uniquely} integrated to a pseudo-group element $\p$ by Theorems \ref{the:extension} and \ref{the:eventual}. This means that each equivalence map $\Lambda:\B^S_p\to\B^{\Sb}_p$ corresponds to a unique pseudo-group element $\p\in\G$ such that $\p\cdot S=\Sb$ so $p$-freeness allows the reduction of the congruence problem to the simpler, finite dimensional problem, of finding all equivalence maps $\Lambda$ of the coframes on $\B^S_p$ and $\B_p^{\Sb}$. When solving this equivalence problem we compute the structure functions of the coframes. If we happen to find structure functions that involve non-normalized pseudo-group parameters we may of course normalize these to obtain a smaller partial moving frame $\B_p^S$ along with a right invariants coframe that determines the equivalence problem. We continue computing structure functions until no more group parameters can be normalized and no new genuine invariants are produced, cf. \cite{olver95}. 
%
%\begin{Rem}\label{rem:upone}
%By the same argument as above, if $\B_q\subset\G_q\iresn$ is any partial moving frame, where $\G$ is hypo-projective, then a map $\Lambda:\B_q^S\to\B_q^{\Sb}$ that preserves the restricted Maurer-Cartan forms $\muaL$, $|L|<q$, gives rise to a (not necessarily unique) pseudo-group element $\p\in\G$ that maps $S$ to $\Sb$.  
%\end{Rem}
%
%The above considerations provide a natural proof of (a generalization of) persistence of freeness of Lie pseudo-groups, see \cite{olver09}.
%
%\begin{theorem}\label{the:persistence}
%Let $\G$ be a Lie pseudo-group of transformations on $\E=\X\times\U$. If all group parameters of order $p$ can be normalized from lifted invariants when restricted to $S\subset\E$, then so can all group parameters of order $p+1$.
%\end{theorem}
%
%\begin{proof}
%As described above we obtain a partial moving frame $\B_p^S$ along with the right invariant coframe $\muaL$, $|L|<p$, that completely determines the equivalence problem. Consider the isotropy (pseudo-)group of $S$ under the action of $\G$. By Cartan's solution of the equivalence problem for coframes this is a finite dimensional local Lie group we shall denote $G$. If we were to move up one order, and consider the partial moving frame $\B_{p+1}^S\subset\G_{p+1}\iresn$ (obtained by taking $(\sigma^{p+1}_p)^{-1}\left(\B_p^S\right)$ and restricting to any $p+1$ normalizations we may have performed) along with the collection of one-forms $\{\muaL\}_{|L|<p+1}$, we can see, by Remark \ref{rem:upone}, that $G$ is precisely the collection of local diffeomorphisms that preserves $\B_{p+1}^S$ and $\{\muaL\}_{|L|<p+1}$. Note that we can write $\B_{p+1}^S$ as the product $\B_p^S\times\H_{p+1}$ where $\H_{p+1}$ is parametrized by the group parameters of order $p+1$ that have not been normalized. Denote these parameters by $y\in\H_{p+1}\subset\R^r$ and let $x\in\B_p^S\subset\R^t$ parametrize $\B_p^S$. When we restrict the Maurer-Cartan forms $\{\muaL\}_{|L|=p}$ to $\B_{p+1}^S=\B_p^S\times\H_{p+1}$ we obtain, since all $p\th$ order group parameters have been normalized, a linear combination of the forms that make up the coframe on $\B_p^S$. The coefficients, $F_i(x,y)$, of this linear combination are invariants of the problem and may depend on $p+1$ order group parameters. Recall that the local Lie group $G$ is the collection of equivalence maps for $\{\muaL\}_{|L|<p}$ on $\B_p^S$ \emph{and} for $\{\muaL\}_{|L|<p+1}$ on $\B_p^S\times\H_{p+1}$. I claim that this implies that all group parameters of order $p+1$ can be normalized in the invariants $F_i(x,y)$. This is a result of the following simple lemma. 
%
%\begin{lemma}
%Let $\pmb{\varpi}=\{\varpi^1, \ldots, \varpi^t\}$ be a local coframe on $\R^t$ with symmetry group $G$. Let $F:\R^t\times\R^r\to\R^v$, $F(x,y)=(F_1(x,y), \ldots, F_v(x,y))$, and assume that the collection of local transformations of $\R^t\times\R^r$ that preserve $\pmb{\varpi}$ and $F$, denoted $\widetilde{G}$, is isomorphic to $G$. Then $\nabla_yF$ is full rank $r$. 
%\end{lemma}
%
%\begin{proof}[Proof of Lemma]
%Note that a transformation $\p\in\widetilde{G}$ must have the form $$\p(x,y)=(\p_1(x), \p_2(x,y)),\quad \p_1:\R^t\to\R^t~~\text{and}~~\p_2:\R^t\times\R^r\to\R^r,$$ where $\p_1\in G$. Since the symmetry groups of $\pmb{\varpi}$ and $\{\pmb{\varpi}, F\}$ are isomorphic the orbits of these two groups in $\R^t$ and $\R^t\times\R^r$ have equal dimensions. By the form of the transformations in $\widetilde{G}$ the orbits of $\widetilde{G}$ in $\R^t\times\R^r$ project to the orbits of $G$ in $\R^t$ and are therefore transverse to the fibration $\R^t\times\R^r\to\R^t$. Since $F$ is constant and has constant rank on each orbit (being invariant) this immediately implies that $\nabla_yF$ is full rank $r$.  
%\end{proof}
%
%Continuing the proof of Theorem \ref{the:persistence}, the invariants we obtain when restricting $\{\muaL\}_{|L|<p+1}$ to $\B_p^S\times\H_{p+1}$ are full rank $\text{dim} ~\H_{p+1}$ in the $p+1$ order group parameters in $\H_{p+1}$. This means that we can normalize all of them.
%
%\end{proof}
%
%


